MiWaves Reinforcement Learning Algorithm

The escalating prevalence of cannabis use poses a significant public health challenge globally. In the U.S., cannabis use is more prevalent among emerging adults (EAs) (ages 18-25) than any other age group, with legalization in the multiple states contributing to a public perception that cannabis is less risky than in prior decades. To address this growing concern, we developed MiWaves, a reinforcement learning (RL) algorithm designed to optimize the delivery of personalized intervention prompts to reduce cannabis use among EAs. MiWaves leverages domain expertise and prior data to tailor the likelihood of delivery of intervention messages. This paper presents a comprehensive overview of the algorithm's design, including key decisions and experimental outcomes. The finalized MiWaves RL algorithm was deployed in a clinical trial from March to May 2024.

==> results.tex <==
\section{Result Tables}
\label{chap:results}
\newgeometry{margin=0.1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 127.5202667 & 1.936879603 & 130.203 & 2.356117781 & 98.80047466 & 4.199041051 & 103.85 & 3.526400431 \\ \hline
        fixed & 0 & 10 & daily & weekly & 127.5254833 & 1.938561799 & 130.23 & 2.316268551 & 98.81337598 & 4.248482869 & 103.87 & 3.539223079 \\ \hline
        fixed & 0 & 20 & daily & daily & 127.76375 & 1.940135081 & 130.527 & 2.474221292 & 98.9621911 & 4.096257991 & 103.9 & 3.356933124 \\ \hline
        fixed & 0 & 20 & daily & weekly & 127.7736 & 1.94593636 & 130.518 & 2.511309619 & 98.98200003 & 4.16376803 & 104.047 & 3.363672249 \\ \hline
        fixed & 1 & 10 & daily & daily & 127.50635 & 1.942291483 & 130.199 & 2.326778674 & 98.82120558 & 4.227405432 & 103.883 & 3.596638848 \\ \hline
        fixed & 1 & 10 & daily & weekly & 127.50555 & 1.935627418 & 130.238 & 2.331384996 & 98.78692887 & 4.266265294 & 103.831 & 3.60776094 \\ \hline
        fixed & 1 & 20 & daily & daily & 127.76605 & 1.951645042 & 130.492 & 2.539869288 & 98.99383578 & 4.096348312 & 103.954 & 3.435095923 \\ \hline
        fixed & 1 & 20 & daily & weekly & 127.7533167 & 1.947932515 & 130.494 & 2.594988247 & 98.99281177 & 4.117442488 & 104.01 & 3.432914214 \\ \hline
        fixed & 2 & 10 & daily & daily & 127.4229 & 1.934572313 & 130.103 & 2.332357391 & 98.68883428 & 4.254044559 & 103.806 & 3.59963387 \\ \hline
        fixed & 2 & 10 & daily & weekly & 127.4247167 & 1.93919508 & 130.103 & 2.357305877 & 98.67887816 & 4.26306528 & 103.809 & 3.626571246 \\ \hline
        fixed & 2 & 20 & daily & daily & 127.7080333 & 1.96247135 & 130.401 & 2.501739195 & 98.95213115 & 4.199555323 & 104.01 & 3.506836181 \\ \hline
        fixed & 2 & 20 & daily & weekly & 127.7016 & 1.962236308 & 130.382 & 2.504411308 & 98.95313689 & 4.187294752 & 104.025 & 3.498839093 \\ \hline
        mixed & 0 & 10 & daily & daily & 128.27465 & 1.987674944 & 131.05 & 2.480423351 & 99.34611146 & 4.210212435 & 104.406 & 3.515560268 \\ \hline
        mixed & 0 & 10 & daily & weekly & 128.25075 & 1.97331007 & 131.051 & 2.459857516 & 99.39725506 & 4.213091823 & 104.474 & 3.508037058 \\ \hline
        mixed & 0 & 20 & daily & daily & 128.5609833 & 1.982196889 & 131.39 & 2.500979808 & 99.54688531 & 4.101317616 & 104.556 & 3.35795533 \\ \hline
        mixed & 0 & 20 & daily & weekly & 128.5357167 & 1.981418056 & 131.371 & 2.581057729 & 99.60042413 & 4.109671566 & 104.539 & 3.519656091 \\ \hline
        mixed & 1 & 10 & daily & daily & 128.3987 & 1.987002413 & 131.194 & 2.52870797 & 99.50635978 & 4.183391204 & 104.484 & 3.57459704 \\ \hline
        mixed & 1 & 10 & daily & weekly & 128.3176167 & 1.98772366 & 131.142 & 2.477263813 & 99.43261222 & 4.213480854 & 104.469 & 3.599241448 \\ \hline
        mixed & 1 & 20 & daily & daily & 128.6402167 & 1.971568674 & 131.449 & 2.525054257 & 99.63167844 & 4.100098793 & 104.599 & 3.444807542 \\ \hline
        mixed & 1 & 20 & daily & weekly & 128.5782833 & 1.97538686 & 131.368 & 2.569936964 & 99.60338645 & 4.106226091 & 104.642 & 3.452656369 \\ \hline
        mixed & 2 & 10 & daily & daily & 128.4906 & 1.999993535 & 131.264 & 2.508247197 & 99.62721972 & 4.237270498 & 104.695 & 3.62359973 \\ \hline
        mixed & 2 & 10 & daily & weekly & 128.3878 & 1.981029416 & 131.233 & 2.522738789 & 99.51207241 & 4.194802487 & 104.664 & 3.507863167 \\ \hline
        mixed & 2 & 20 & daily & daily & 128.8154667 & 1.973368863 & 131.65 & 2.644522641 & 99.80259064 & 4.189101554 & 104.753 & 3.556612293 \\ \hline
        mixed & 2 & 20 & daily & weekly & 128.7537333 & 1.995443687 & 131.536 & 2.597056796 & 99.76804943 & 4.17815131 & 104.765 & 3.580820437 \\ \hline
    \end{tabular}
    \caption{Minimal effect environment}
    \label{tab:minimal_effect}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 128.56465 & 1.904596695 & 131.19 & 2.110900282 & 100.6089116 & 4.386561835 & 105.776 & 3.791414512 \\ \hline
        fixed & 0 & 10 & daily & weekly & 128.5718 & 1.892089977 & 131.178 & 2.10506912 & 100.5829436 & 4.372708546 & 105.751 & 3.825767766 \\ \hline
        fixed & 0 & 20 & daily & daily & 129.1122667 & 1.878121572 & 131.854 & 2.157008113 & 101.3098728 & 4.284163988 & 106.559 & 3.701488755 \\ \hline
        fixed & 0 & 20 & daily & weekly & 129.0970833 & 1.863672068 & 131.84 & 2.204177851 & 101.3183966 & 4.239233376 & 106.595 & 3.713014274 \\ \hline
        fixed & 1 & 10 & daily & daily & 128.57155 & 1.892352053 & 131.19 & 2.109004504 & 100.5956421 & 4.381221704 & 105.759 & 3.793075138 \\ \hline
        fixed & 1 & 10 & daily & weekly & 128.5657333 & 1.905087696 & 131.144 & 2.109327855 & 100.5867411 & 4.373058989 & 105.741 & 3.817645741 \\ \hline
        fixed & 1 & 20 & daily & daily & 129.1326167 & 1.842475814 & 131.915 & 2.207549546 & 101.3803502 & 4.172473154 & 106.557 & 3.60960538 \\ \hline
        fixed & 1 & 20 & daily & weekly & 129.1289833 & 1.864497577 & 131.877 & 2.250860058 & 101.3651582 & 4.246888031 & 106.56 & 3.761834659 \\ \hline
        fixed & 2 & 10 & daily & daily & 128.45805 & 1.897579175 & 131.097 & 2.154087046 & 100.3613767 & 4.381829935 & 105.674 & 3.830499184 \\ \hline
        fixed & 2 & 10 & daily & weekly & 128.4603167 & 1.900472846 & 131.11 & 2.160763754 & 100.3589705 & 4.368914657 & 105.684 & 3.787234347 \\ \hline
        fixed & 2 & 20 & daily & daily & 129.09925 & 1.93275318 & 131.853 & 2.320105817 & 101.2195398 & 4.351398761 & 106.547 & 3.723746903 \\ \hline
        fixed & 2 & 20 & daily & weekly & 129.10805 & 1.905204146 & 131.846 & 2.29396687 & 101.2045932 & 4.32948651 & 106.588 & 3.726158343 \\ \hline
        mixed & 0 & 10 & daily & daily & 129.0586167 & 1.912850782 & 131.79 & 2.194060163 & 101.1167889 & 4.351942983 & 106.37 & 3.781018381 \\ \hline
        mixed & 0 & 10 & daily & weekly & 129.02565 & 1.916161599 & 131.716 & 2.144374967 & 101.0451626 & 4.368294618 & 106.217 & 3.811877621 \\ \hline
        mixed & 0 & 20 & daily & daily & 129.43705 & 1.913621623 & 132.285 & 2.292220539 & 101.5169859 & 4.317297695 & 106.8 & 3.729209031 \\ \hline
        mixed & 0 & 20 & daily & weekly & 129.4411167 & 1.891547383 & 132.28 & 2.253131155 & 101.5760933 & 4.253998209 & 106.837 & 3.709168505 \\ \hline
        mixed & 1 & 10 & daily & daily & 129.1124667 & 1.898319176 & 131.856 & 2.158069508 & 101.1874894 & 4.338993282 & 106.41 & 3.902678567 \\ \hline
        mixed & 1 & 10 & daily & weekly & 129.0699333 & 1.908092895 & 131.802 & 2.172278988 & 101.1341157 & 4.381919451 & 106.408 & 3.881692414 \\ \hline
        mixed & 1 & 20 & daily & daily & 129.4525667 & 1.900600584 & 132.268 & 2.276878565 & 101.5646372 & 4.30222862 & 106.82 & 3.764518562 \\ \hline
        mixed & 1 & 20 & daily & weekly & 129.4494667 & 1.905467424 & 132.251 & 2.263735629 & 101.6261122 & 4.295028609 & 106.933 & 3.723440747 \\ \hline
        mixed & 2 & 10 & daily & daily & 129.155 & 1.9083 & 131.915 & 2.228289703 & 101.2987667 & 4.282975003 & 106.523 & 3.740049599 \\ \hline
        mixed & 2 & 10 & daily & weekly & 129.0658833 & 1.91571841 & 131.805 & 2.231473728 & 101.1283752 & 4.329366497 & 106.42 & 3.768899043 \\ \hline
        mixed & 2 & 20 & daily & daily & 129.5678 & 1.90865524 & 132.448 & 2.284796709 & 101.7180931 & 4.31932701 & 106.945 & 3.812279502 \\ \hline
        mixed & 2 & 20 & daily & weekly & 129.5371 & 1.908891616 & 132.41 & 2.293229164 & 101.6978916 & 4.34416145 & 106.99 & 3.798802443 \\ \hline
    \end{tabular}
    \label{tab:low_effect}
    \caption{Low treatment effect environment}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 128.0302833 & 1.926506194 & 130.516 & 2.13886512 & 99.85784746 & 4.36592651 & 104.984 & 3.875015355 \\ \hline
        fixed & 0 & 10 & daily & weekly & 128.0407833 & 1.919231161 & 130.507 & 2.11150444 & 99.84922638 & 4.392646253 & 104.969 & 3.828124737 \\ \hline
        fixed & 0 & 20 & daily & daily & 128.4229667 & 1.896490041 & 130.976 & 2.2517602 & 100.2938701 & 4.240917451 & 105.447 & 3.706843806 \\ \hline
        fixed & 0 & 20 & daily & weekly & 128.411 & 1.883084674 & 130.973 & 2.240484546 & 100.3325364 & 4.255496013 & 105.446 & 3.78180962 \\ \hline
        fixed & 1 & 10 & daily & daily & 128.0235 & 1.914119169 & 130.512 & 2.099013101 & 99.7506776 & 4.341390913 & 104.818 & 3.753381942 \\ \hline
        fixed & 1 & 10 & daily & weekly & 128.0287333 & 1.914780001 & 130.482 & 2.13744614 & 99.81296485 & 4.380672877 & 104.939 & 3.89162935 \\ \hline
        fixed & 1 & 20 & daily & daily & 128.4430167 & 1.861707843 & 130.994 & 2.238071491 & 100.2595886 & 4.202812591 & 105.402 & 3.639422482 \\ \hline
        fixed & 1 & 20 & daily & weekly & 128.4332667 & 1.878243786 & 131.016 & 2.258482676 & 100.3417825 & 4.220598502 & 105.425 & 3.695656234 \\ \hline
        fixed & 2 & 10 & daily & daily & 127.9276333 & 1.909188603 & 130.453 & 2.158539089 & 99.56885039 & 4.401338755 & 104.76 & 3.799657879 \\ \hline
        fixed & 2 & 10 & daily & weekly & 127.9275333 & 1.913038007 & 130.47 & 2.161504106 & 99.56046986 & 4.401899333 & 104.75 & 3.779484092 \\ \hline
        fixed & 2 & 20 & daily & daily & 128.3962833 & 1.916948224 & 130.993 & 2.287236542 & 100.2759603 & 4.287441322 & 105.456 & 3.72653512 \\ \hline
        fixed & 2 & 20 & daily & weekly & 128.3861167 & 1.911242659 & 130.976 & 2.249538619 & 100.2353508 & 4.349347823 & 105.427 & 3.785785387 \\ \hline
        mixed & 0 & 10 & daily & daily & 128.4628833 & 1.925569322 & 131.027 & 2.261585948 & 100.2593186 & 4.338881892 & 105.383 & 3.775289525 \\ \hline
        mixed & 0 & 10 & daily & weekly & 128.4376167 & 1.927438459 & 131.012 & 2.211301879 & 100.2626609 & 4.320337241 & 105.402 & 3.709365984 \\ \hline
        mixed & 0 & 20 & daily & daily & 128.7624 & 1.929992981 & 131.423 & 2.318959034 & 100.5985229 & 4.240593899 & 105.711 & 3.595271756 \\ \hline
        mixed & 0 & 20 & daily & weekly & 128.7657 & 1.916785984 & 131.393 & 2.285618297 & 100.6340826 & 4.242558175 & 105.795 & 3.722831584 \\ \hline
        mixed & 1 & 10 & daily & daily & 128.5013167 & 1.929268446 & 131.129 & 2.249413035 & 100.3154797 & 4.308970506 & 105.439 & 3.874245604 \\ \hline
        mixed & 1 & 10 & daily & weekly & 128.4816333 & 1.932090664 & 131.048 & 2.199248963 & 100.3143719 & 4.352119129 & 105.448 & 3.820379039 \\ \hline
        mixed & 1 & 20 & daily & daily & 128.7699833 & 1.925801557 & 131.396 & 2.302212849 & 100.6243774 & 4.23018943 & 105.749 & 3.682322501 \\ \hline
        mixed & 1 & 20 & daily & weekly & 128.7936333 & 1.900177848 & 131.403 & 2.286501913 & 100.6717943 & 4.287534009 & 105.861 & 3.680785106 \\ \hline
        mixed & 2 & 10 & daily & daily & 128.5234833 & 1.927367824 & 131.191 & 2.248114543 & 100.3073281 & 4.307814306 & 105.491 & 3.786082276 \\ \hline
        mixed & 2 & 10 & daily & weekly & 128.4509 & 1.912021261 & 131.019 & 2.257241458 & 100.3071092 & 4.297714893 & 105.435 & 3.823516052 \\ \hline
        mixed & 2 & 20 & daily & daily & 128.8969667 & 1.936070037 & 131.561 & 2.345587133 & 100.8340403 & 4.243750506 & 105.899 & 3.678899156 \\ \hline
        mixed & 2 & 20 & daily & weekly & 128.8449667 & 1.916584041 & 131.508 & 2.296287438 & 100.7298509 & 4.274400799 & 105.833 & 3.753080202 \\ \hline
    \end{tabular}
    \caption{Low effect environment with decaying treatment effect}
    \label{tab:low_effect_decay}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 130.9748167 & 1.86769238 & 134.32 & 1.99138143 & 104.071333 & 4.511324641 & 109.477 & 3.957141772 \\ \hline
        fixed & 0 & 10 & daily & weekly & 130.96265 & 1.843464162 & 134.269 & 1.974876958 & 104.0717954 & 4.437781934 & 109.468 & 3.888698497 \\ \hline
        fixed & 0 & 20 & daily & daily & 132.2153667 & 1.80917023 & 135.875 & 2.13280918 & 105.3391949 & 4.452608221 & 110.728 & 3.962450757 \\ \hline
        fixed & 0 & 20 & daily & weekly & 132.2098333 & 1.823621846 & 135.906 & 2.165909509 & 105.3808289 & 4.407400488 & 110.702 & 3.987128791 \\ \hline
        fixed & 1 & 10 & daily & daily & 130.9791667 & 1.825302905 & 134.262 & 1.921290192 & 104.0254454 & 4.438628183 & 109.401 & 3.903549539 \\ \hline
        fixed & 1 & 10 & daily & weekly & 130.9656667 & 1.833565546 & 134.227 & 1.934675942 & 104.0650884 & 4.437062424 & 109.471 & 3.911222188 \\ \hline
        fixed & 1 & 20 & daily & daily & 132.2699333 & 1.832303467 & 135.868 & 2.122163047 & 105.4308197 & 4.374157796 & 110.728 & 3.946266083 \\ \hline
        fixed & 1 & 20 & daily & weekly & 132.2713 & 1.810906059 & 135.903 & 2.115441089 & 105.444803 & 4.34839868 & 110.829 & 3.923424397 \\ \hline
        fixed & 2 & 10 & daily & daily & 130.9047833 & 1.866905352 & 134.257 & 2.079050504 & 103.7866259 & 4.504404744 & 109.291 & 3.880955939 \\ \hline
        fixed & 2 & 10 & daily & weekly & 130.89675 & 1.856301915 & 134.256 & 2.04266101 & 103.7723038 & 4.53260281 & 109.276 & 3.905742439 \\ \hline
        fixed & 2 & 20 & daily & daily & 132.5320167 & 1.873798968 & 136.178 & 2.236138636 & 105.6410925 & 4.4677894 & 111.083 & 3.988560016 \\ \hline
        fixed & 2 & 20 & daily & weekly & 132.5268167 & 1.853178997 & 136.186 & 2.203044257 & 105.6492529 & 4.438961404 & 111.096 & 4.066790381 \\ \hline
        mixed & 0 & 10 & daily & daily & 131.5756167 & 1.850681266 & 134.95 & 2.03997549 & 104.5288132 & 4.444746419 & 110.03 & 3.931806201 \\ \hline
        mixed & 0 & 10 & daily & weekly & 131.5663 & 1.833846331 & 135.002 & 2.04058717 & 104.623757 & 4.376603512 & 110.085 & 3.956548369 \\ \hline
        mixed & 0 & 20 & daily & daily & 132.24815 & 1.84410496 & 135.802 & 2.094945345 & 105.285354 & 4.36966402 & 110.718 & 3.873819304 \\ \hline
        mixed & 0 & 20 & daily & weekly & 132.2454167 & 1.826565377 & 135.832 & 2.044939119 & 105.2945553 & 4.431187195 & 110.744 & 3.927399139 \\ \hline
        mixed & 1 & 10 & daily & daily & 131.6430833 & 1.842852203 & 135.085 & 2.039430067 & 104.6751973 & 4.424284031 & 110.112 & 3.939474077 \\ \hline
        mixed & 1 & 10 & daily & weekly & 131.5829667 & 1.852886451 & 135.012 & 2.010436768 & 104.6140012 & 4.435060422 & 110.118 & 3.985232239 \\ \hline
        mixed & 1 & 20 & daily & daily & 132.2089333 & 1.836186545 & 135.757 & 2.081694262 & 105.2367909 & 4.428373419 & 110.588 & 3.913726613 \\ \hline
        mixed & 1 & 20 & daily & weekly & 132.2368667 & 1.830676261 & 135.751 & 2.072799797 & 105.2894484 & 4.440577028 & 110.726 & 3.966096822 \\ \hline
        mixed & 2 & 10 & daily & daily & 131.7671 & 1.878747982 & 135.214 & 2.039657814 & 104.8230966 & 4.469202191 & 110.265 & 4.042186908 \\ \hline
        mixed & 2 & 10 & daily & weekly & 131.6786 & 1.856851677 & 135.132 & 2.044401135 & 104.7448117 & 4.481995538 & 110.166 & 4.081475714 \\ \hline
        mixed & 2 & 20 & daily & daily & 132.4677 & 1.833894168 & 136.025 & 2.031471142 & 105.4967134 & 4.372894997 & 110.931 & 3.972749552 \\ \hline
        mixed & 2 & 20 & daily & weekly & 132.4468 & 1.845362064 & 136.031 & 2.126861302 & 105.4533215 & 4.450138756 & 110.945 & 4.066383528 \\ \hline
    \end{tabular}
    \caption{High treatment effect environment}
    \label{tab:high_effect}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 129.2956833 & 1.867291444 & 132.058 & 2.098007626 & 101.6822244 & 4.402777239 & 107.012 & 3.865987067 \\ \hline
        fixed & 0 & 10 & daily & weekly & 129.29575 & 1.864167261 & 132.051 & 2.068308246 & 101.7201202 & 4.460920449 & 107.004 & 3.968120966 \\ \hline
        fixed & 0 & 20 & daily & daily & 130.05165 & 1.82191838 & 132.995 & 2.219115815 & 102.6365827 & 4.221101081 & 107.955 & 3.734497958 \\ \hline
        fixed & 0 & 20 & daily & weekly & 130.0608833 & 1.817986607 & 133.036 & 2.268414424 & 102.6162015 & 4.22034705 & 107.988 & 3.747113022 \\ \hline
        fixed & 1 & 10 & daily & daily & 129.2873333 & 1.860790782 & 132.042 & 2.087878349 & 101.6744255 & 4.319062788 & 106.94 & 3.757179793 \\ \hline
        fixed & 1 & 10 & daily & weekly & 129.2946667 & 1.860833415 & 132.007 & 2.072305721 & 101.6545698 & 4.403578752 & 106.931 & 3.852497761 \\ \hline
        fixed & 1 & 20 & daily & daily & 130.0656333 & 1.829951514 & 132.992 & 2.272649555 & 102.6673084 & 4.207670553 & 108.009 & 3.728326568 \\ \hline
        fixed & 1 & 20 & daily & weekly & 130.0895333 & 1.810998851 & 133.048 & 2.251598543 & 102.6082106 & 4.21584615 & 107.936 & 3.788390687 \\ \hline
        fixed & 2 & 10 & daily & daily & 129.2094 & 1.862852569 & 132.04 & 2.155550974 & 101.5451951 & 4.414821639 & 106.872 & 3.935557902 \\ \hline
        fixed & 2 & 10 & daily & weekly & 129.21225 & 1.866923812 & 132.036 & 2.138621986 & 101.5281992 & 4.436456387 & 106.865 & 3.954525888 \\ \hline
        fixed & 2 & 20 & daily & daily & 130.1972 & 1.855327223 & 133.181 & 2.344939018 & 102.7267171 & 4.31754172 & 108.153 & 3.790526481 \\ \hline
        fixed & 2 & 20 & daily & weekly & 130.1979333 & 1.854675295 & 133.201 & 2.314540775 & 102.7981992 & 4.265208879 & 108.211 & 3.761379933 \\ \hline
        mixed & 0 & 10 & daily & daily & 129.7807833 & 1.886797779 & 132.625 & 2.162377164 & 102.1972515 & 4.322761956 & 107.608 & 3.889259055 \\ \hline
        mixed & 0 & 10 & daily & weekly & 129.7587833 & 1.865264114 & 132.642 & 2.197916286 & 102.17208 & 4.326272188 & 107.524 & 3.812928533 \\ \hline
        mixed & 0 & 20 & daily & daily & 130.2218833 & 1.881976468 & 133.136 & 2.19556462 & 102.7615501 & 4.325501685 & 108.014 & 3.783358825 \\ \hline
        mixed & 0 & 20 & daily & weekly & 130.2295833 & 1.840045657 & 133.228 & 2.182662594 & 102.7509544 & 4.332597023 & 108.036 & 3.852233638 \\ \hline
        mixed & 1 & 10 & daily & daily & 129.8447667 & 1.88316868 & 132.694 & 2.193938012 & 102.340561 & 4.329570809 & 107.673 & 3.852735522 \\ \hline
        mixed & 1 & 10 & daily & weekly & 129.7741333 & 1.847348573 & 132.634 & 2.161953746 & 102.1762983 & 4.329915243 & 107.515 & 3.763811233 \\ \hline
        mixed & 1 & 20 & daily & daily & 130.25405 & 1.883020951 & 133.141 & 2.263982995 & 102.739656 & 4.310955876 & 108.122 & 3.833551356 \\ \hline
        mixed & 1 & 20 & daily & weekly & 130.2415167 & 1.834590964 & 133.181 & 2.227496128 & 102.738184 & 4.31682777 & 108.098 & 3.876647521 \\ \hline
        mixed & 2 & 10 & daily & daily & 129.9133833 & 1.882101566 & 132.781 & 2.17291026 & 102.3855356 & 4.368588845 & 107.775 & 3.95460175 \\ \hline
        mixed & 2 & 10 & daily & weekly & 129.8320667 & 1.873644193 & 132.717 & 2.191668542 & 102.3367839 & 4.343566353 & 107.762 & 3.876384398 \\ \hline
        mixed & 2 & 20 & daily & daily & 130.4123333 & 1.864605886 & 133.34 & 2.265921446 & 102.9131327 & 4.245663645 & 108.239 & 3.827189439 \\ \hline
        mixed & 2 & 20 & daily & weekly & 130.4183833 & 1.867313124 & 133.414 & 2.259779635 & 102.9702834 & 4.314311684 & 108.271 & 3.839408678 \\ \hline
    \end{tabular}
    \caption{High treatment effect environment with decaying treatment effect}
    \label{tab:high_effect_decay}
\end{table}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 129.76835 & 1.881535152 & 132.706 & 2.047575151 & 102.3847955 & 4.455428352 & 107.729 & 3.884721226 \\ \hline
        fixed & 0 & 10 & daily & weekly & 129.782 & 1.864947989 & 132.745 & 2.030634137 & 102.3838773 & 4.498396099 & 107.717 & 3.900180893 \\ \hline
        fixed & 0 & 20 & daily & daily & 130.6570667 & 1.845485876 & 133.86 & 2.167579295 & 103.4207466 & 4.362566218 & 108.816 & 3.851122434 \\ \hline
        fixed & 0 & 20 & daily & weekly & 130.6431 & 1.83783452 & 133.858 & 2.206543904 & 103.4381302 & 4.343043175 & 108.846 & 3.755167639 \\ \hline
        fixed & 1 & 10 & daily & daily & 129.7624833 & 1.871794927 & 132.722 & 2.03880259 & 102.3556584 & 4.472211625 & 107.647 & 3.873356555 \\ \hline
        fixed & 1 & 10 & daily & weekly & 129.78355 & 1.865925026 & 132.759 & 2.045340803 & 102.3744657 & 4.489988147 & 107.737 & 3.921521516 \\ \hline
        fixed & 1 & 20 & daily & daily & 130.71 & 1.837883822 & 133.903 & 2.174187434 & 103.4872325 & 4.28879016 & 108.913 & 3.698909434 \\ \hline
        fixed & 1 & 20 & daily & weekly & 130.7059167 & 1.845069667 & 133.904 & 2.194717294 & 103.5581742 & 4.286657358 & 108.919 & 3.734024504 \\ \hline
        fixed & 2 & 10 & daily & daily & 129.5837167 & 1.888901942 & 132.582 & 2.112883338 & 101.9709591 & 4.394546474 & 107.311 & 3.829070253 \\ \hline
        fixed & 2 & 10 & daily & weekly & 129.5890167 & 1.885824033 & 132.582 & 2.155522211 & 101.9880338 & 4.38897747 & 107.381 & 3.83005731 \\ \hline
        fixed & 2 & 20 & daily & daily & 130.7063167 & 1.876082788 & 133.948 & 2.31631086 & 103.3683777 & 4.319933574 & 108.867 & 3.74457087 \\ \hline
        fixed & 2 & 20 & daily & weekly & 130.7193167 & 1.871134921 & 133.933 & 2.302826741 & 103.3879877 & 4.303600156 & 108.899 & 3.756101569 \\ \hline
        mixed & 0 & 10 & daily & daily & 130.3114333 & 1.883377389 & 133.411 & 2.134848707 & 102.9420296 & 4.417937062 & 108.393 & 3.871827863 \\ \hline
        mixed & 0 & 10 & daily & weekly & 130.2904167 & 1.890980263 & 133.402 & 2.135742494 & 102.9623676 & 4.417237231 & 108.348 & 3.756181039 \\ \hline
        mixed & 0 & 20 & daily & daily & 130.8205 & 1.877307328 & 134.024 & 2.197139959 & 103.4795485 & 4.348806757 & 108.897 & 3.843942117 \\ \hline
        mixed & 0 & 20 & daily & weekly & 130.83275 & 1.880027872 & 134.021 & 2.208859208 & 103.5408374 & 4.361230384 & 108.903 & 3.764318132 \\ \hline
        mixed & 1 & 10 & daily & daily & 130.3690667 & 1.883758821 & 133.448 & 2.133376666 & 102.9719219 & 4.370886474 & 108.35 & 3.82994778 \\ \hline
        mixed & 1 & 10 & daily & weekly & 130.30945 & 1.879089467 & 133.313 & 2.111760166 & 102.9506045 & 4.395436407 & 108.283 & 3.850637739 \\ \hline
        mixed & 1 & 20 & daily & daily & 130.8305167 & 1.872318448 & 134.018 & 2.1949205 & 103.4972467 & 4.416865068 & 108.932 & 3.803074546 \\ \hline
        mixed & 1 & 20 & daily & weekly & 130.8325333 & 1.873698415 & 134.045 & 2.177722434 & 103.5043896 & 4.364008348 & 108.906 & 3.863180555 \\ \hline
        mixed & 2 & 10 & daily & daily & 130.3718167 & 1.8784631 & 133.485 & 2.185240261 & 103.0133187 & 4.343862829 & 108.518 & 3.920417835 \\ \hline
        mixed & 2 & 10 & daily & weekly & 130.2864 & 1.87336552 & 133.369 & 2.180215356 & 102.976222 & 4.317690009 & 108.424 & 3.787904962 \\ \hline
        mixed & 2 & 20 & daily & daily & 130.9633333 & 1.868423801 & 134.141 & 2.217345034 & 103.6597847 & 4.315968882 & 109.045 & 3.820795074 \\ \hline
        mixed & 2 & 20 & daily & weekly & 130.9154333 & 1.850653603 & 134.14 & 2.239955357 & 103.5702053 & 4.323787876 & 109.048 & 3.863896479 \\ \hline
    \end{tabular}
    \caption{Environment with low treatment effect in the morning, and high treatment effect in the evening}
    \label{tab:morning_low_eve_high}
\end{table}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 128.61045 & 1.899999808 & 131.211 & 2.109734343 & 100.6840459 & 4.359102442 & 105.934 & 3.774207731 \\ \hline
        fixed & 0 & 10 & daily & weekly & 128.6152833 & 1.888941695 & 131.239 & 2.05508613 & 100.6567781 & 4.365270098 & 105.869 & 3.86889377 \\ \hline
        fixed & 0 & 20 & daily & daily & 129.1632333 & 1.852328007 & 131.898 & 2.2238696 & 101.4459796 & 4.217904711 & 106.723 & 3.757628374 \\ \hline
        fixed & 0 & 20 & daily & weekly & 129.1639333 & 1.859009152 & 131.96 & 2.201908263 & 101.3744459 & 4.264045003 & 106.652 & 3.733483092 \\ \hline
        fixed & 1 & 10 & daily & daily & 128.6062333 & 1.89278272 & 131.241 & 2.098194224 & 100.6823344 & 4.408896922 & 105.904 & 3.906505344 \\ \hline
        fixed & 1 & 10 & daily & weekly & 128.6237167 & 1.898926347 & 131.234 & 2.096960658 & 100.7108366 & 4.443301881 & 105.916 & 3.93280358 \\ \hline
        fixed & 1 & 20 & daily & daily & 129.19495 & 1.856800989 & 131.925 & 2.25496674 & 101.447005 & 4.220517493 & 106.739 & 3.741440765 \\ \hline
        fixed & 1 & 20 & daily & weekly & 129.1807 & 1.864298724 & 131.894 & 2.238696942 & 101.4479447 & 4.233524527 & 106.671 & 3.729914074 \\ \hline
        fixed & 2 & 10 & daily & daily & 128.4905333 & 1.900669281 & 131.136 & 2.159746281 & 100.4304642 & 4.435781273 & 105.754 & 3.899933846 \\ \hline
        fixed & 2 & 10 & daily & weekly & 128.4942833 & 1.9088286 & 131.15 & 2.174511439 & 100.430449 & 4.39942433 & 105.753 & 3.850388422 \\ \hline
        fixed & 2 & 20 & daily & daily & 129.1804667 & 1.883665636 & 131.909 & 2.318236183 & 101.3492145 & 4.271149746 & 106.661 & 3.682740691 \\ \hline
        fixed & 2 & 20 & daily & weekly & 129.1751333 & 1.896973242 & 131.905 & 2.350420175 & 101.2770392 & 4.266893573 & 106.578 & 3.737501304 \\ \hline
        mixed & 0 & 10 & daily & daily & 129.0790667 & 1.900925466 & 131.846 & 2.189128594 & 101.1435676 & 4.360358166 & 106.445 & 3.770341496 \\ \hline
        mixed & 0 & 10 & daily & weekly & 129.05085 & 1.91912074 & 131.77 & 2.16981566 & 101.1346997 & 4.401271321 & 106.344 & 3.879518527 \\ \hline
        mixed & 0 & 20 & daily & daily & 129.4537167 & 1.894543977 & 132.223 & 2.256495291 & 101.6622261 & 4.275679827 & 106.925 & 3.761100238 \\ \hline
        mixed & 0 & 20 & daily & weekly & 129.4350667 & 1.896580342 & 132.186 & 2.218423765 & 101.6261055 & 4.25158001 & 106.927 & 3.730974538 \\ \hline
        mixed & 1 & 10 & daily & daily & 129.1311833 & 1.899539408 & 131.807 & 2.242822106 & 101.284705 & 4.348645104 & 106.521 & 3.871570612 \\ \hline
        mixed & 1 & 10 & daily & weekly & 129.0598 & 1.900508211 & 131.742 & 2.20305152 & 101.1992494 & 4.351677888 & 106.457 & 3.874874321 \\ \hline
        mixed & 1 & 20 & daily & daily & 129.4619833 & 1.898437262 & 132.264 & 2.252843537 & 101.6802397 & 4.271564869 & 106.945 & 3.611159786 \\ \hline
        mixed & 1 & 20 & daily & weekly & 129.4475833 & 1.87761584 & 132.257 & 2.294439147 & 101.5964791 & 4.254712825 & 106.811 & 3.790881032 \\ \hline
        mixed & 2 & 10 & daily & daily & 129.15335 & 1.89593777 & 131.852 & 2.269822901 & 101.2758608 & 4.234305229 & 106.53 & 3.815769909 \\ \hline
        mixed & 2 & 10 & daily & weekly & 129.0657333 & 1.906019985 & 131.78 & 2.239553527 & 101.2059333 & 4.284115335 & 106.43 & 3.800539435 \\ \hline
        mixed & 2 & 20 & daily & daily & 129.5791333 & 1.882282782 & 132.387 & 2.277439571 & 101.813489 & 4.241696769 & 107.071 & 3.787011883 \\ \hline
        mixed & 2 & 20 & daily & weekly & 129.5355167 & 1.88782851 & 132.338 & 2.269968282 & 101.7407641 & 4.23505979 & 106.98 & 3.693453668 \\ \hline
    \end{tabular}
    \caption{Environment with low treatment effect in the morning, and high treatment effect in the evening - and decaying treatment effect across time}
    \label{tab:morning_low_eve_high_decay}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 129.79235 & 1.854219724 & 132.726 & 2.031729313 & 102.3957094 & 4.446305418 & 107.716 & 3.829796861 \\ \hline
        fixed & 0 & 10 & daily & weekly & 129.7771333 & 1.842549307 & 132.723 & 1.98815769 & 102.4054458 & 4.410396427 & 107.722 & 3.852235195 \\ \hline
        fixed & 0 & 20 & daily & daily & 130.6511333 & 1.808692927 & 133.874 & 2.124882114 & 103.4817532 & 4.330618093 & 108.816 & 3.770164983 \\ \hline
        fixed & 0 & 20 & daily & weekly & 130.6477833 & 1.816143565 & 133.835 & 2.183409032 & 103.4634806 & 4.326323784 & 108.866 & 3.764046227 \\ \hline
        fixed & 1 & 10 & daily & daily & 129.7768667 & 1.846208837 & 132.719 & 2.049033675 & 102.3960291 & 4.452847119 & 107.639 & 3.832776931 \\ \hline
        fixed & 1 & 10 & daily & weekly & 129.7622167 & 1.846094693 & 132.726 & 2.046686102 & 102.378938 & 4.355636207 & 107.644 & 3.764208283 \\ \hline
        fixed & 1 & 20 & daily & daily & 130.6809167 & 1.811507006 & 133.871 & 2.131398367 & 103.4774194 & 4.316929615 & 108.794 & 3.789665421 \\ \hline
        fixed & 1 & 20 & daily & weekly & 130.68075 & 1.827870838 & 133.897 & 2.14240309 & 103.5431187 & 4.286959332 & 108.927 & 3.730170371 \\ \hline
        fixed & 2 & 10 & daily & daily & 129.5825667 & 1.864125717 & 132.568 & 2.112907002 & 102.0100607 & 4.392198769 & 107.354 & 3.788493632 \\ \hline
        fixed & 2 & 10 & daily & weekly & 129.58415 & 1.87970019 & 132.587 & 2.157065368 & 102.0025816 & 4.432741144 & 107.35 & 3.869173038 \\ \hline
        fixed & 2 & 20 & daily & daily & 130.7011833 & 1.870674378 & 133.877 & 2.332674645 & 103.4513345 & 4.305457622 & 108.911 & 3.781213959 \\ \hline
        fixed & 2 & 20 & daily & weekly & 130.7157167 & 1.859903391 & 133.858 & 2.335987157 & 103.4617237 & 4.276449287 & 108.991 & 3.694782673 \\ \hline
        mixed & 0 & 10 & daily & daily & 130.29185 & 1.874266181 & 133.366 & 2.146868417 & 102.9345937 & 4.346667157 & 108.255 & 3.854928663 \\ \hline
        mixed & 0 & 10 & daily & weekly & 130.2771167 & 1.85850301 & 133.393 & 2.061807702 & 102.9242129 & 4.350577382 & 108.279 & 3.8054775 \\ \hline
        mixed & 0 & 20 & daily & daily & 130.83755 & 1.848510624 & 134.043 & 2.175695521 & 103.5513777 & 4.272182361 & 108.918 & 3.729111959 \\ \hline
        mixed & 0 & 20 & daily & weekly & 130.83795 & 1.844570318 & 134.074 & 2.204205979 & 103.5867275 & 4.31427721 & 108.949 & 3.758443694 \\ \hline
        mixed & 1 & 10 & daily & daily & 130.3504333 & 1.866900084 & 133.459 & 2.136075607 & 102.9653021 & 4.355672667 & 108.317 & 3.808807031 \\ \hline
        mixed & 1 & 10 & daily & weekly & 130.2799333 & 1.863966081 & 133.337 & 2.115403271 & 102.9255601 & 4.379203924 & 108.315 & 3.904519817 \\ \hline
        mixed & 1 & 20 & daily & daily & 130.8103167 & 1.848347711 & 134.035 & 2.212300838 & 103.5557387 & 4.251139292 & 108.946 & 3.735248854 \\ \hline
        mixed & 1 & 20 & daily & weekly & 130.82165 & 1.847422311 & 133.995 & 2.229007627 & 103.5535702 & 4.338500638 & 108.945 & 3.823934492 \\ \hline
        mixed & 2 & 10 & daily & daily & 130.3805 & 1.85997671 & 133.484 & 2.162809284 & 103.0181646 & 4.326213738 & 108.386 & 3.825703073 \\ \hline
        mixed & 2 & 10 & daily & weekly & 130.3188833 & 1.874856351 & 133.38 & 2.126640543 & 103.0049213 & 4.385020031 & 108.389 & 3.83981497 \\ \hline
        mixed & 2 & 20 & daily & daily & 130.9351333 & 1.856892366 & 134.104 & 2.225799632 & 103.5775774 & 4.318142026 & 109.005 & 3.783183184 \\ \hline
        mixed & 2 & 20 & daily & weekly & 130.92025 & 1.856792581 & 134.058 & 2.209442464 & 103.57403 & 4.407128899 & 108.883 & 3.935455628 \\ \hline
    \end{tabular}
    \caption{Environment with high treatment effect in the morning, and low treatment effect in the evening}
    \label{tab:morning_high_eve_low}
\end{table}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{0.05\linewidth}|p{0.05\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|p{0.06\linewidth}|}
    \hline
        \textbf{Reward model Variant} & \textbf{Baseline and Advantage Variant} & \textbf{Smooth allocation function variant (value of B)} & \textbf{Posterior Update Cadence} & \textbf{Hyper Update Cadence} & \textbf{Mean Avg total reward per user} & \textbf{Std Avg total reward per user} & \textbf{Mean of Avg Median} & \textbf{Std of Avg Median} & \textbf{[Lower 25] Mean Avg total reward per user} & \textbf{[Lower 25] Std Avg total reward per user} & \textbf{[Lower 25] Mean of Avg Median} & \textbf{[Lower 25] Std of Avg Median} \\ \hline \hline
        fixed & 0 & 10 & daily & daily & 128.7124833 & 1.875722935 & 131.364 & 2.113410514 & 100.8614081 & 4.350779738 & 106.095 & 3.812804086 \\ \hline
        fixed & 0 & 10 & daily & weekly & 128.7076 & 1.870428654 & 131.315 & 2.121620843 & 100.8454358 & 4.342045877 & 106.066 & 3.799031982 \\ \hline
        fixed & 0 & 20 & daily & daily & 129.2844833 & 1.83345884 & 132.099 & 2.248043371 & 101.5018961 & 4.235582011 & 106.699 & 3.682648368 \\ \hline
        fixed & 0 & 20 & daily & weekly & 129.2828833 & 1.826183997 & 132.101 & 2.219526751 & 101.5449649 & 4.257065902 & 106.778 & 3.729170953 \\ \hline
        fixed & 1 & 10 & daily & daily & 128.6977833 & 1.878903109 & 131.305 & 2.11907409 & 100.8460568 & 4.3583912 & 106.076 & 3.814737737 \\ \hline
        fixed & 1 & 10 & daily & weekly & 128.6931333 & 1.877354023 & 131.301 & 2.100928128 & 100.8399688 & 4.333898963 & 106.061 & 3.792595286 \\ \hline
        fixed & 1 & 20 & daily & daily & 129.2890833 & 1.845386024 & 132.077 & 2.207843065 & 101.5710596 & 4.273294217 & 106.698 & 3.72206878 \\ \hline
        fixed & 1 & 20 & daily & weekly & 129.29795 & 1.834299395 & 132.135 & 2.231204831 & 101.5298151 & 4.242629715 & 106.699 & 3.718588307 \\ \hline
        fixed & 2 & 10 & daily & daily & 128.5746667 & 1.882089752 & 131.227 & 2.14335508 & 100.5936633 & 4.409143073 & 105.886 & 3.871176049 \\ \hline
        fixed & 2 & 10 & daily & weekly & 128.5705167 & 1.882604589 & 131.21 & 2.136796668 & 100.6094458 & 4.411460226 & 105.911 & 3.904174561 \\ \hline
        fixed & 2 & 20 & daily & daily & 129.2860833 & 1.880626763 & 132.072 & 2.306906153 & 101.4971573 & 4.269890471 & 106.775 & 3.714683701 \\ \hline
        fixed & 2 & 20 & daily & weekly & 129.2899 & 1.864051275 & 132.075 & 2.29496732 & 101.5080137 & 4.262971024 & 106.766 & 3.712848502 \\ \hline
        mixed & 0 & 10 & daily & daily & 129.1618167 & 1.893714224 & 131.889 & 2.180637292 & 101.316622 & 4.367707604 & 106.507 & 3.879104407 \\ \hline
        mixed & 0 & 10 & daily & weekly & 129.1361833 & 1.896979123 & 131.89 & 2.179885318 & 101.2975307 & 4.321331639 & 106.55 & 3.884906691 \\ \hline
        mixed & 0 & 20 & daily & daily & 129.5333833 & 1.891204458 & 132.311 & 2.234005148 & 101.6988122 & 4.295287601 & 106.976 & 3.827195318 \\ \hline
        mixed & 0 & 20 & daily & weekly & 129.5502833 & 1.858263243 & 132.342 & 2.230254694 & 101.778646 & 4.229229404 & 106.946 & 3.726806139 \\ \hline
        mixed & 1 & 10 & daily & daily & 129.20575 & 1.884995025 & 131.967 & 2.182982135 & 101.3569711 & 4.338748127 & 106.55 & 3.849870128 \\ \hline
        mixed & 1 & 10 & daily & weekly & 129.1607167 & 1.880304427 & 131.904 & 2.22031169 & 101.3834302 & 4.264791824 & 106.622 & 3.769232813 \\ \hline
        mixed & 1 & 20 & daily & daily & 129.55635 & 1.867859317 & 132.329 & 2.240593448 & 101.797286 & 4.280387915 & 107.018 & 3.792581706 \\ \hline
        mixed & 1 & 20 & daily & weekly & 129.5522333 & 1.871420884 & 132.384 & 2.255558467 & 101.8092904 & 4.259771436 & 107.043 & 3.817807093 \\ \hline
        mixed & 2 & 10 & daily & daily & 129.2401 & 1.906940042 & 131.998 & 2.228227098 & 101.4375415 & 4.323851919 & 106.67 & 3.767638518 \\ \hline
        mixed & 2 & 10 & daily & weekly & 129.16215 & 1.894473986 & 131.848 & 2.232912 & 101.373105 & 4.311451021 & 106.629 & 3.883665665 \\ \hline
        mixed & 2 & 20 & daily & daily & 129.6458 & 1.873374443 & 132.431 & 2.254493069 & 101.8889139 & 4.268795264 & 107.194 & 3.806752422 \\ \hline
        mixed & 2 & 20 & daily & weekly & 129.6534833 & 1.884791679 & 132.465 & 2.250838733 & 101.9001885 & 4.271248223 & 107.059 & 3.801054985 \\ \hline
    \end{tabular}
    \caption{Environment with high treatment effect in the morning, and low treatment effect in the evening - and decaying treatment effect across time}
    \label{tab:morning_high_eve_low_decay}
\end{table}


\end{landscape}

